Fiducial Inference and Decision Theory

The majority of the statisticians concluded many decades ago that fiducial inference was nonsensical to them. Hannig et al. (2016) and others have, however, contributed to a renewed interest and focus. Fiducial inference is similar to Bayesian analysis, but without requiring a prior. The prior information is replaced by assuming a particular data generating equation. Berger (1985) explains that Bayesian analysis and statistical decision theory are in harmony. Taraldsen and Lindqvist (2013) show that fiducial theory and statistical decision theory also play well together. The purpose of this text is to explain and exemplify this together with recent mathematical results.

==> def.tex <==
% def.tex
% 12/2-1991 (def.tex)
% 1998-06-15 15:08 (Fjerner IKKE AMS versjoner)
% 2004-01-15 19:52 (aoscm test)
% 2004-04-01 21:53 (elsart)

\newcommand{\vekk}[1]{}

\usepackage[utf8]{inputenc}
\RequirePackage[OT1]{fontenc}

%\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}

% Conflicts? \usepackage{url}
\RequirePackage{natbib}
%\usepackage[ISBN=false,url=false,doi=false,style=chicago]{biblatex}
%\usepackage[backend=biber,ISBN=false,url=false,doi=false,style=chicago]{biblatex}
%\addbibresource{JABREFgtaralds.bib}

%\RequirePackage{amsthm,amsmath}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
% \usepackage{theorem}

\usepackage{orcidlink}
% \usepackage{doi}

%\usepackage[a4paper]{geometry}
\usepackage[a4paper,includeheadfoot,margin=2.54cm]{geometry}
%\usepackage[top=1in, bottom=1.25in, left=1.25in, right=1.25in]{geometry}

\usepackage{tikz-cd}

\newtheorem{Def}{Definition}
\newtheorem{prop}{Proposition}
\newtheorem{theo}{Theorem}
\newtheorem{example}{Example}


% My commands

\newcommand{\QED}{$\square$}
%\newcommand{\QED}{$\square$}
\newcommand{\idx}[1]{#1}


\newcommand{\thetaml}{\hat{\theta}_{\text{\tiny ML}}}
\newcommand{\thetamu}{\hat{\theta}_{\text{\tiny MU}}}

\newcommand{\forallp}{\forall} % sometimes with prime ...

\newcommand{\gG}{\operatorname{G}} % A group

\newcommand{\pU}{\operatorname{\hat{U}}} % parameter generating U
\newcommand{\pV}{\operatorname{\hat{V}}} % parameter generating V

\newcommand{\Sstat}{\operatorname{S}} % p-value stat
\newcommand{\C}{\operatorname{C}} % Confidence distribution
\newcommand{\K}{\operatorname{K}} % Confidence distribution
\newcommand{\N}{\operatorname{N}} % Confidence net
%\newcommand{\K}{\operatorname{{\cal{K}}}} % Confidence distribution
\newcommand{\plev}{\text{\it p}} % Confidence level

\newcommand{\Renyi}{Rényi }

\newcommand{\LossI}{L_{\textrm{I}}} % ...
\newcommand{\LossII}{L_{\textrm{II}}} % ... 

\newcommand{\lik}{=} % ... 

\newcommand{\darrow}{\overset{D}{\rightarrow}} % 

\newcommand{\halpha}{\hat{\alpha}} % 
\newcommand{\hbeta}{\hat{\beta}} % 

\newcommand{\ttau}{\tilde{\tau}} % 
\newcommand{\htau}{\hat{\tau}} % 
\newcommand{\tv}{\tilde{v}} % 
\newcommand{\hv}{\hat{v}} % 
\newcommand{\hw}{\hat{w}} % 
\newcommand{\tw}{\tilde{w}} % 
\newcommand{\htheta}{\hat{\theta}} % 
\newcommand{\ttheta}{\tilde{\theta}} % 

\newcommand{\ceps}{{\cal E}} % a sigma field
\newcommand{\cB}{{\cal B}} % a sigma field
\newcommand{\ca}{{\cal A}} % an Algebra
\newcommand{\cF}{{\cal F}} % an Algebra
\newcommand{\cE}{{\cal E}} % an Algebra
\newcommand{\cG}{{\cal G}} % an Algebra
\newcommand{\cT}{{\cal T}} % an Algebra

\newcommand{\cL}{{\ell}} % Loss

\newcommand{\barx}{\bar{x}} % 

\newcommand{\Si}{\operatorname{Si}} % The Sine integral function

\newcommand{\binorm}{\operatorname{binormal}}
\newcommand{\Cov}{\operatorname{Cov}}
%\newcommand{\Var}{\operatorname{Var}}


\newcommand{\Pow}{\operatorname{Pow}} % Power
\newcommand{\pr}{\operatorname{P}} % Probability
\renewcommand{\Pr}{\operatorname{P}} % Probability
%\renewcommand{\Pr}{\operatorname{Pr}} % Probability
%\renewcommand{\Pr}{\operatorname{P}} % Probability
%\newcommand{\pr}{\operatorname{pr}} % Probability
%\newcommand{\pr}{\operatorname{\text{P}}} % Probability
\newcommand{\var}{\operatorname{var}} % Probability
\newcommand{\Std}{\operatorname{Std}} % std
\newcommand{\E}{{\operatorname{\text{E}}}} % Expectation
\newcommand{\Prob}{\mathord{\mbox{$P$}}} % Expectation

\newcommand{\setX}{{\text{\bf X}}} % A set X
\newcommand{\setT}{{\text{\bf T}}} % A set X
\newcommand{\setB}{{\text{\bf B}}} % A set X


\newcommand{\bset}{\Omega} % basic probability space
\newcommand{\bevents}{{\cal E}} % basic probability space

\newcommand{\bmu}{{\boldsymbol{\mu}}} % random variable
\newcommand{\bsigma}{{\boldsymbol{\sigma}}} % 
\newcommand{\bx}{{\boldsymbol{x}}} % 
\newcommand{\bv}{{\boldsymbol{v}}} % 
\newcommand{\br}{{\boldsymbol{r}}} % 

\newcommand{\bbchi}{{\boldsymbol{\chi}}} %
\newcommand{\bbp}{{\boldsymbol{p}}} % 
\newcommand{\bbs}{{\boldsymbol{s}}} % 
\newcommand{\bbu}{{\boldsymbol{u}}} % 
\newcommand{\bbv}{{\boldsymbol{v}}} % 
\newcommand{\bbw}{{\boldsymbol{w}}} % 
\newcommand{\bbT}{{\boldsymbol{T}}} % 
\newcommand{\bbpi}{{\boldsymbol{\pi}}} % 
\newcommand{\bbn}{{\boldsymbol{n}}} % 
\newcommand{\bbx}{{\boldsymbol{x}}} % 
\newcommand{\bby}{{\boldsymbol{y}}} % 
\newcommand{\bbt}{{\boldsymbol{t}}} % 
\newcommand{\bbr}{{\boldsymbol{r}}} % 
\newcommand{\bbz}{{\boldsymbol{z}}} % 
\newcommand{\bbtheta}{{\boldsymbol{\theta}}} % 
\newcommand{\bbsigma}{{\boldsymbol{\sigma}}} % 
\newcommand{\bbrho}{{\boldsymbol{\rho}}} % 

\newcommand{\half}{\frac{1}{2}} % half!

\newcommand{\HMean}[1]{\widetilde{#1}} % harmonic mean. Check ISO!

\newcommand{\m}{\operatorname{m}}
\newcommand{\mb}{\operatorname{M}}

\newcommand{\abs}[1]{\left| #1 \right|} 
%\newcommand{\Div}{\mathop{div}} 
%\newcommand{\curl}{\mathop{curl}} 
%\newcommand{\dlik}{\mathop{:=}\nolimits} 
%\newcommand{\E}{\operatorname{E}}
\newcommand{\Grad}{\mathop{\text{grad}}} 
%\newcommand{\into}{\mbox{$\: \rightarrow \:$}} 
%\renewcommand{\P}{\operatorname{P}}
\newcommand{\RealN}{{\mbox{$\mathbb R$}}} % Real numbers
\newcommand{\st}{\operatornamewithlimits{{\mid}}}
%\newcommand{\supp}{\mathop{\mbox{supp}}}
\newcommand{\Tr}{\mathop{\text{tr}}\nolimits} 
%\newcommand{\V}{\operatorname{Var}}

% Orddeling
% \hyphenation{ana-ly-sen}

\newcommand{\IG}{\mathop{IG}} % Inverse Gaussian
\newcommand{\Wald}{\mathop{Wald}} % Inverse Gaussian
\newcommand{\Normal}{\mathop{\text{N}}} % Normal, or Gaussian
\newcommand{\Uniform}{\mathop{Uniform}} % Uniform
\newcommand{\U}{\mathop{\text{U}}} % Uniform
\newcommand{\B}{\mathop{\text{\bf B}}} % Binom and Bernoulli
\newcommand{\Beta}{\mathop{\text{Beta}}} % Beta

\newcommand{\Pareto}{\mathop{\text{Pareto}}} % Beta

\newcommand{\normvar}{\mathop{\bf N}}
\newcommand{\gamvar}{\mathop{\bf Gamma}}
\newcommand{\betavar}{\mathop{\bf Beta}}
\newcommand{\expvar}{\mathop{\bf Exp}}
\newcommand{\chitwovar}{\mathop{\bf \chi^2}}
\newcommand{\dirvar}{\mathop{\bf Dir}}
\newcommand{\univar}{\mathop{\bf U}}


% SI units
\newcommand{\SIm}{\text{m}} % meter
\newcommand{\SIcm}{\text{cm}} % centi meter
\newcommand{\SIs}{\text{s}} % seconds


% New commands
\newcommand{\hatt}{\hat{\theta}}
\newcommand{\Lloc}{L_{1,\text{loc}}}
%\newcommand{\E}{\mathop{\rm E}} % Expectation
%\newcommand{\E}{\mathop{\text{E}}} % Expectation
%\newcommand{\E}{\mathop{\mbox{$\Bbb E$}}} % Expectation


%\newcommand{\e}{\rm e} % 2.7...
\newcommand{\M}{\mathord{m}}
\newcommand{\s}{\mathord{s}}

%\newcommand{\C}{\mathord{\cal C}}
\newcommand{\W}{\mathord{\cal W}}

\newcommand{\AW}{\mathord{{\hat{W}_A}}}
\newcommand{\AS}{\mathord{{S_A}}}
\newcommand{\AzDelta}{\mathord{{\Delta_{Az}}}}
\newcommand{\ADelta}{\mathord{{\Delta_{A}}}}

\newcommand{\BW}{\mathord{{\hat{W}_B}}}
\newcommand{\BtW}{\mathord{{\tilde{W}_B}}}
\newcommand{\BS}{\mathord{{S_B}}}
\newcommand{\BDelta}{\mathord{{\Delta_B}}}

%\DeclareMathOperator*{\Fhyp}{F}

\newcommand{\nc}{\newcommand}
\nc{\beqns}{\begin{eqnarray*}}
\nc{\eeqns}{\end{eqnarray*}}
\nc{\beqn}{\begin{eqnarray}}
\nc{\eeqn}{\end{eqnarray}}
\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\newcommand{\bes}{ \begin{equation} \begin{split} } %Nummerert slutt.
\newcommand{\ees}{ \end{split} \end{equation} } %Nummerert slutt.

\newcommand{\ii}{\mbox{\boldmath $\imath$}} % \sqrt{-1}
\newcommand{\beeq}[1]{\label{\knavn #1}} 
\newcommand{\be}[1]{\begin{equation}\label{eq#1}} 
\newcommand{\ee}{\end{equation}}%Nummerert slutt.
\newcommand{\eg}{{\it e g }}
\newcommand{\de}[1]{\stackrel{(\ref{\knavn #1})}{=}}
\newcommand{\id}{\mathop{id}}
\newcommand{\im}{\mathop{\mbox{Im}}\nolimits}
\newcommand{\Kg}{\mathord{kg}}
\newcommand{\li}[1]{{#1}\!-\!\lim\;}
\newcommand{\nn}{{nearest neighbor}}
\newcommand{\no}{\mathop{\mbox{\#}}\nolimits}
\newcommand{\Pa}{\mathord{Pa}}
\newcommand{\Hi}{ {\cal H} }
\newcommand{\gr}{\mathop{|}}
\newcommand{\hd}{\hat{\delta}}
\newcommand{\re}{\mathop{\mbox{Re}}\nolimits}
\newcommand{\Sc}{{S}chr{\"o}dinger\ }
\newcommand{\so}{{S}chr{\"o}dinger\ }
%\newcommand{\tr}{\mathop{\mbox{tr}}\nolimits}
%\newcommand{\Tr}{\mathop{\mbox{Tr}}\nolimits}

\newcommand{\alf}{Alf Taraldsen }                       
\newcommand{\bra}[1]{\left \langle #1 \right. |}
\newcommand{\COp}{{\cal C}} 
\newcommand{\der}[2]{ \frac{\partial #1}{\partial #2} }%Derivert.
\newcommand{\del}{\mathop{\triangle}}
\newcommand{\Div}{\mathop{\text{div}}}
\newcommand{\Ess}{\mathop{\mbox{Ess}}}
\newcommand{\etc}{{etc}} % et cetera, and the rest
\newcommand{\iid}{{i.i.d. }}
\newcommand{\Lin}{\mathop{\mbox{Lin}}}
\newcommand{\mto}{{\em mto}\ }
\newcommand{\pot}{{\cal P}}
\newcommand{\sgn}{\mathop{\mbox{sgn}}\nolimits} %Fortegnsfunksjon.      
\newcommand{\ess}{\mathop{\mbox{ess}}\nolimits}                 
\newcommand{\ket}[1]{\left. | #1 \right \rangle}
\newcommand{\Var}{\mathop{\mbox{Var}}\nolimits} % Variance

\newcommand{\curl}{\mathop{curl}\nolimits} 
%\newcommand{\dlik}{\stackrel{def}{=}}                          %Fire tegn.
\newcommand{\diam}{\mathop{\mbox{diam}}\nolimits} 
\newcommand{\dlik}{\mathop{=}\nolimits} % since := etc can be avoided ... 
\newcommand{\fpar}[1]{\left [ #1 \right ]}
\newcommand{\fsum}{\mathop{\dot{+}}} % 1992-07-28 17:38
% \newcommand{\Grad}{\mathop{\mbox{\bf grad}}}
%\newcommand{\half}{\frac{1}{2}} 
\newcommand{\IntN}{{\mbox{$\bf Z$}}} % Integers
\newcommand{\into}{\mbox{$\: \rightarrow \:$}} 
\newcommand{\konj}[1]{\overline{#1}}
\newcommand{\kpar}[1]{\left \{#1\right \}}
\newcommand{\likd}{\mathop{=:}\nolimits} 
\newcommand{\lims}{\mathop{\overline{\lim}\;}}
\newcommand{\limi}{\mathop{\underline{\lim}\;}}
\newcommand{\llim}{\mathop{l\!-\!\lim\;}}
\newcommand{\lsum}{\mathop{\hat{+}}} % 1992-07-28 17:08
\newcommand{\maxm}{m_{\text{max}}}
\newcommand{\mean}[1]{\left \langle#1 \right \rangle }
\newcommand{\NatN}{{\mbox{$\Bbb N$}}} % Natural numbers: 1, 2, ...
\newcommand{\norm}[1]{\left \| #1\right\|}
\newcommand{\nlim}{\mathop{n\!-\!\lim\;}}
\newcommand{\plim}{\mathop{p\!-\!\lim\;}}
\newcommand{\refl}[1]{(\ref{\knavn #1})} 
\newcommand{\refp}[1]{\refl{#1} p\aa\ side \pageref{#1}}  %Anngir og side.
\newcommand{\rpar}[1]{\left (#1\right )}                
\newcommand{\RatN}{{\mbox{$\Bbb Q$}}} % Rational numbers
\newcommand{\Real}{{\mbox{$\Bbb R$}}} % Real numbers\mbox{$\Bbb C$}
\newcommand{\slim}{\mathop{s\!-\!\lim\;}}
\newcommand{\supp}{\mathop{\mbox{supp}}}
\newcommand{\ulim}{\mathop{u\!-\!\lim\;}}
\newcommand{\vlim}{\mathop{v\!-\!\lim\;}}
\newcommand{\wlim}{\mathop{w\!-\!\lim\;}}
\newcommand{\Vlim}{\mathop{V\!-\!\lim\;}}
\newcommand{\Didx}[1]{\index{#1}}

%\newcommand{\CompN}{{\mbox{$\bf C$}}}
\newcommand{\CompN}{{\mbox{$\Bbb C$}}}                           %Fem
\newcommand{\QuartN}{{\mbox{$\Bbb H$}}}
\newcommand{\OctN}{{\mbox{$\Bbb O$}}}  
\newcommand{\compl}{\mathop{\sim}}
\newcommand{\gtdef}[1]{{\em #1}}
\newcommand{\imply}{\Rightarrow}
\newcommand{\lkpar}[1]{\left\{ \begin{array}{ll} #1 \end{array}\right.}
\newcommand{\Lclim}{\mathop{L_c\!-\!\lim\;}}
\newcommand{\Lilim}{\mathop{L_i\!-\!\lim\;}}
\newcommand{\Lmlim}{\mathop{L_m\!-\!\lim\;}}
\newcommand{\pplus}{\dot{+}}
\newcommand{\Uclim}{\mathop{U_c\!-\!\lim\;}}
\newcommand{\Umlim}{\mathop{U_m\!-\!\lim\;}}
\newcommand{\uclim}{\mathop{\tilde{u}\!-\!\lim\;}}
\newcommand{\uthev}[1]{{\it #1}}
\newcommand{\Vclim}{\mathop{\tilde{V}\!-\!\lim\;}}
\newcommand{\vclim}{\mathop{\tilde{v}\!-\!\lim\;}}
%\newcommand{\RealN}{{\mbox{$\Bbb R$}}} % Real numbers
\newcommand{\csigma}{{\tilde{\sigma}}}

\newcommand{\braket}[2]{\left \langle #1 | #2 \right \rangle }
\newcommand{\figtxt}{\footnotesize} % Size on figure texts
\newcommand{\hanche}{Harald \mbox{Hanche-Olsen} }
\newcommand{\holden}{Helge Holden }
\newcommand{\sarrow}{\stackrel{s}{\rightarrow}}
%\newcommand{\setdif}{\bigtriangleup}
\newcommand{\warrow}{\stackrel{w}{\rightarrow}}

\newcommand{\Complex}{\mbox{$\bf C$}}
\newcommand{\martens}{Henrik Martens }
\newcommand{\svektor}[2]{\fpar{\begin{array}{cc} #1\\#2 \end{array} }} %Vektor.

\newcommand{\rsvektor}[2]{\left .\begin{array}{ccc}
&\multicolumn{2}{c}{#1}\\
&\multicolumn{2}{c}{#2}\end{array} \right ]} %Stor matrise,
\newcommand{\lsvektor}[2]{\left [\begin{array}{c} #1,\\#2,\end{array}\right .} %Stor matrise.


